Quantum Neural Networks under Depolarization Noise: Exploring White-Box Attacks and Defenses

Leveraging the unique properties of quantum mechanics, Quantum Machine Learning (QML) promises computational breakthroughs and enriched perspectives where traditional systems reach their boundaries. However, similarly to classical machine learning, QML is not immune to adversarial attacks. Quantum adversarial machine learning has become instrumental in highlighting the weak points of QML models when faced with adversarial crafted feature vectors. Diving deep into this domain, our exploration shines light on the interplay between depolarization noise and adversarial robustness. While previous results enhanced robustness from adversarial threats through depolarization noise, our findings paint a different picture. Interestingly, adding depolarization noise discontinued the effect of providing further robustness for a multi-class classification scenario. Consolidating our findings, we conducted experiments with a multi-class classifier adversarially trained on gate-based quantum simulators, further elucidating this unexpected behavior.

==> inputs/amplitude_embedding.tex <==
\begin{array}{c}
\textbf{Amplitude Embedding} +  \\
\textbf{Strongly Entangling Layers} \\
\end{array}

==> inputs/stronglyentangling.tex <==
\begin{array}{c}
     \textbf{Strongly Entangling Layers}
     \\
     \\
       \overbrace{\includegraphics[width=0.4\textwidth]{img/strongly_ent_layer_circ.pdf}}^{\times \ \text{Nr. Layers}}
\end{array}

==> sections/discussion.tex <==
For the iris dataset, adversarial training, randomized smoothing, and the addition of depolarization noise all proved to increase the robustness of the model. 
However, this trend was discontinued when these techniques were tested on the MNIST dataset. 
It is important to recognize that the QNN used in this work compared to classical neural networks lacks of capacity.
Nevertheless, it highlights the importance of scaling QML architectures and concepts to larger datasets.
Additionally, we see a discrepancy between the known advantages of depolarization noise on a small dataset scaled to a larger one.
We see one future work direction on towards increasing the capacity of the network we used for MNIST, to circumvent the disagreement faced. Hereby the work of \cite{9643575} could be a helpful tool. 
Additionally most, robustness methods are tested on even larger datasets, we plan to further incoperate the diverse datasets into our work.

==> sections/structure.tex <==
\begin{itemize}
    \item Background
    
    \begin{itemize}
        \item Quantum
        information basics
            \begin{itemize}
                \item Noise: Depolarization, bit-flip, phase-Flip
            \end{itemize}
        \item Quantum machine learning
        \begin{itemize}
            \item encoding
            \item 
        \end{itemize} 
        \item Quantum neural networks (Nicola)
        \begin{itemize}
            \item hybrid: convolutional, pulling reference
        \end{itemize}
        \item Adversarial Robustness (Nicola)
        \begin{itemize}
            \item Gradient-based attacks (PGD, FGSM), blackbox, ...
            \item Also possible on the quantum side
        \end{itemize}
        \item Certified Robustness
            \begin{itemize}
                \item Quantum Hypothesis Test (add reference to randomized smoothing)
                \item Quadro,
                \item Lipschitz
            \end{itemize}
    \end{itemize}
    \item Related Work
        \begin{itemize}
            \item Weber et. al \cite{Weber_2021}
            \item QQ Approaches 
            \item QuAdRo (Nicola)
            \item Some classicals (Nicola)
        \end{itemize}
        
    \item Methods
    
    \begin{itemize}
        \item Data-preprocessing
        \item Model structure, why we choose it
        \item Simulation description, runtime, ...
        \item Explain upperbound on trace distance
    \end{itemize}
    \item Experiments
    
    \begin{itemize}
        \item Iris
        \begin{itemize}
            \item Same pattern as Du et. al 
            \item Comparison of PGD adversarial training, random smoothing
        \end{itemize}
        \item MNIST-2
        \begin{itemize}
            \item compare depolarization noise towards random smooth, pgd, ...
            \item Best results for depolarization norm
            \item Min upperbound is positive
        \end{itemize}
        \item MNIST-4
        \begin{itemize}
            \item compare depolarization noise towards random smooth, pgd, ...
            \item Best results for depolarization norm
            \item Min upper-bound is negative: immediate adveresarial example present (model structure?)
        \end{itemize}
        \item MNIST-10
        \begin{itemize}
            \item compare depolarization noise towards random smooth, pgd, ...
            \item Best results for depolarization norm
            \item Min upper-bound is negative: immediate adveresarial example present (model structure?)
        \end{itemize}
    \end{itemize}
    \item Conclustion
    \begin{itemize}
        \item Reasons
    \end{itemize}
\end{itemize}


Research Questions


\begin{itemize}
    \item RQ1: How is the performance of depolarization noise for a multi-class classifier?
    \begin{itemize}
        \item Plot the three vanilla plots: zero to even a negative effect
        \item Explanation: Models capacity
        \item Explanation: Minimal trace distance among the quantum states (dep will increase prob. of follow-up)
    \end{itemize}
    \item RQ2: How do other adversarial training strategies perform on our networks?
    \begin{itemize}
        \item Neither provide a good performance
        \item TODO which is best?
        \item Same Explanation...
    \end{itemize}
    \item RQ3: How does adding deplolarization noise interact with adversarial training
    \begin{itemize}
        \item Little ot no effect on MNIST2
    \end{itemize}
\end{itemize}
